Mitigating Word Bias in Zero-shot Prompt-based Classifiers

Prompt-based classifiers are an attractive approach for zero-shot classification. However, the precise choice of the prompt template and label words can largely influence performance, with semantically equivalent settings often showing notable performance difference. This discrepancy can be partly attributed to word biases, where the classifier may be biased towards classes. To address this problem, it is possible to optimise classification thresholds on a labelled data set, however, this mitigates some of the advantages of prompt-based classifiers. This paper instead approaches this problem by examining the expected marginal probabilities of the classes. Here, probabilities are reweighted to have a uniform prior over classes, in an unsupervised fashion. Further, we draw a theoretical connection between the class priors and the language models' word prior, and offer the ability to set a threshold in a zero-resource fashion. We show that matching class priors correlates strongly with the oracle upper bound performance and demonstrate large consistent performance gains for prompt settings over a range of NLP tasks.

==> acl_old.tex <==
% % This must be in the first 5 lines to tell arXiv to use pdfLaTeX, which is strongly recommended.
% \pdfoutput=1
% % In particular, the hyperref package requires pdfLaTeX in order to break URLs across lines.

% \documentclass[11pt]{article}

% % Remove the "review" option to generate the final version.
% \usepackage[review]{acl}
% % \usepackage{acl}

% % Standard package includes
% \usepackage{times}
% \usepackage{latexsym}

% % For proper rendering and hyphenation of words containing Latin characters (including in bib files)
% \usepackage[T1]{fontenc}
% % For Vietnamese characters
% % \usepackage[T5]{fontenc}
% % See https://www.latex-project.org/help/documentation/encguide.pdf for other character sets

% % My packages
% \usepackage{bm}
% \usepackage{bbm}
% \usepackage{amssymb} %ge lt

% % This assumes your files are encoded as UTF8
% \usepackage[utf8]{inputenc}

% % This is not strictly necessary, and may be commented out,
% % but it will improve the layout of the manuscript,
% % and will typically save some space.
% \usepackage{microtype}

% %% Useful packages
% \usepackage{amsmath}
% \usepackage{graphicx}
% % \usepackage[colorlinks=true, allcolors=blue]{hyperref}
% % \usepackage[colorinlistoftodos]{todonotes}
% \usepackage{float}
% \usepackage{subcaption}
% \usepackage{amsfonts}
% \usepackage{multicol}
% \usepackage[bottom]{footmisc}
% \usepackage{booktabs}
% \usepackage{multirow}

% % \newcommand{\cev}[1]{\reflectbox{\ensuremath{\vec{\reflectbox{\ensuremath{#1}}}}}}
% % \setlength{\columnseprule}{0.4pt}
% \usepackage{pifont}% http://ctan.org/pkg/pifont
% \newcommand{\cmark}{\ding{51}}%
% \newcommand{\xmark}{\ding{55}}%
% \newcommand{\br}[1]{\bm{\mathrm{#1}}}
% \newcommand{\std}[1]{\scriptsize{$\pm$#1}}
% \newcommand{\argmax}[1]{\underset{#1}{\text{argmax}}\;}
% \newcommand{\argmin}[1]{\underset{#1}{\text{argmin}}\;}

% % \DeclareMathOperator*{\argmax}{arg\,max}
% % \DeclareMathOperator*{\argmin}{arg\,min}
% % \newcommand{\norm}[1]{\left\lVert#1\right\rVert}

% % If the title and author information does not fit in the area allocated, uncomment the following
% %
% %\setlength\titlebox{<dim>}
% %
% % and set <dim> to something 5cm or larger.

% \title{Mitigating Word Bias in Zero-shot Prompt-based Classifiers}
% %\title{Implicit Word Biases in Prompt-based Classifiers}

% %Eliciting meaningful class probabilities from prompted LLMs

% % Author information can be set in various styles:
% % For several authors from the same institution:
% % \author{Author 1 \and ... \and Author n \\
% %         Address line \\ ... \\ Address line}
% % if the names do not fit well on one line use
% %         Author 1 \\ {\bf Author 2} \\ ... \\ {\bf Author n} \\
% % For authors from different institutions:
% % \author{Author 1 \\ Address line \\  ... \\ Address line
% %         \And  ... \And
% %         Author n \\ Address line \\ ... \\ Address line}
% % To start a seperate ``row'' of authors use \AND, as in
% % \author{Author 1 \\ Address line \\  ... \\ Address line
% %         \AND
% %         Author 2 \\ Address line \\ ... \\ Address line \And
% %         Author 3 \\ Address line \\ ... \\ Address line}

% \author{Adian Liusie, Potsawee Manakul, Mark J. F. Gales \\
%   Department of Engineering, University of Cambridge \\
%   \texttt{al826@cam.ac.uk, pm574@cam.ac.uk, mjfg@eng.cam.ac.uk}}


% \begin{document}
% \pagenumbering{arabic}
% \pagestyle{plain}
% \maketitle
% \begin{abstract}
%     %Prompt-based classifiers are an attractive zero-shot approach of zero-shot classification. However, there is a known sensitivity to design choices such as the prompt template and label words. It is highly desired for these systems to be robust, such that most sensible settings work well across a range of tasks. This work analyses different classifier settings and demonstrates that using unlabelled task data to account for the inherent bias leads to greater robustness. We show large consistent gains in prompt settings over a range of NLP tasks and illustrate that many settings which initially fail can be made effective through a simple re-weighting of probabilities. We further show that matching class priors correlates strongly with the oracle upper bound performance, and draw a theoretical relationship connecting class biases with the word priors of the label words, which we use to motivate a zero-resource method of accounting for bias.

%     % Prompt-based classifiers are an attractive approach for zero-shot classification. However, performance is sensitive to the precise choice of the prompt template and label words. To address this problem it is possible to optimise classification thresholds on a labelled development set, mitigating some of the advantages of prompt-based classifiers. This paper approaches this problem by examining the expected probabilities of the classes. Here classification thresholds are derived in terms of expected probabilities. Now a dataset labelled for the specific task of interest is not needed, only examples of the text inputs that need to be classified and the class priors. This probability can be further approximated as the large language model word prior to offer the ability to set a threshold in a zero-shot fashion. We demonstrate that matching class priors correlates strongly with the oracle upper bound performance and demonstrate large consistent gains in prompt settings over a range of NLP tasks. This illustrates that many settings which initially fail can be made effective through a simple re-weighting of probabilities, where the unlabeled inputs are 
    
%     Prompt-based classifiers are an attractive approach for zero-shot classification. However, the precise choice of the prompt template and label words can largely influence performance, with semantically equivalent settings often showing notable performance difference. This discrepancy can be partly attributed to word biases, where the classifier may be biased towards classes. To address this problem, it is possible to optimise classification thresholds on a labelled data set, however, this mitigates some of the advantages of prompt-based classifiers. This paper instead approaches this problem by examining the expected marginal probabilities of the classes. Here, probabilities are reweighted to have a uniform prior over classes, in an unsupervised fashion. Further, we draw a theoretical connection between the class priors and the language models' word prior, and offer the ability to set a threshold in a zero-resource fashion. We show that matching class priors correlates strongly with the oracle upper bound performance and demonstrate large consistent performance gains for prompt settings over a range of NLP tasks.
% \end{abstract}



% \section{Introduction}
% Large language models (LLM) have shown impressive general ability for natural language processing (NLP) tasks. LLMs can effectively handle a range of NLP tasks through ‘prompting’, where a natural language instruction is added to the input, conditioning the model to the task at hand. Prompting can either be an emergent ability learned through scaling up model size \cite{brown2020language, wei2022emergent} or an ability learned through instruction tuning \cite{weifinetuned, chung2022scaling, ouyang2022training}. Despite the recent popularity of prompting, there is a known sensitivity of prompt-based LLMs to elements such as prompt template and label words \cite{gao2021making, schick2021exploiting}. Previous works have demonstrated that prompt templates can significantly impact task performance \citep{shin2020autoprompt, zhou2022large} and that factors such as chosen label words can influence system performance for classification tasks \citep{zhao2021calibrate, holtzman2021surface} %, with factors such as label word’s frequency in the training data shown to impact output decisions.

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/diagram.pdf}
%     \caption{Instead of using the raw LM output probabilities of the label words, we consider mitigating bias by finding weights that make the classifier unbiased over classes. This is connected to normalising by word priors, which we use as a zero-resource de-biasing approach}
%     \label{fig:my_label}
% \end{figure}

% This work focuses on the influence of `word biases' for prompt-based classifiers. i.e. the bias that prompts may have towards certain classes, independent of the input text. To account for this bias, one could use a labelled dataset to find optimal class decision thresholds. This, however, requires labelled task data, which may limit the zero-shot benefits of prompt-based classifiers. We propose a simple unsupervised solution of re-weighting probabilities, where we use unlabelled data to search for weight parameters that ensure a uniform prior over classes. We show that this prior matching leads to greater robustness for diverse prompt settings and that the unsupervised weights which debias the classifier is highly correlated with the oracle weights that maximise accuracy. Further, we provide theoretical analysis that draws a connection between word priors and inherent class bias, which we use to motivate a zero-resource normalisation approach that is competitive with prior matching. Overall, we demonstrate that our unsupervised approach highly reduces sensitivity to the chosen prompt and label words, and that settings which initially fail can often be made effective through a simple probability re-weighting.

% Our contributions are 1) We propose a simple unsupervised probability re-weighting method, and empirically demonstrate greater robustness to prompt and label word choice, with large accuracy gains across prompt settings for a range of standard NLP tasks. 2) We theoretically connect the weight parameters to word priors and use this to motivate a zero-resource re-weighting approach. 3) We show that the weights of prior matching are highly correlated with the optimal oracle weights that maximize accuracy, illustrating that our approach is a near-optimal use of a system's output probabilities. 

% \section{Mitigiating Bias by Re-weighting}
% \textbf{Prompt-based classifiers} Given an input sequence, LMs model the probability distribution over possible output sequences, $P_{\theta}(\br{w}|\br{x})$. For classification task $\mathcal{T}$, a prompt-based classifier comprises of the prompt  $\br{p}$ which reformats the input text $\br{x}\in\mathcal{X}$ to $\br{p}(\br{x})\in\mathcal{X}$ and class words $\{w_i\}_{1:N}$ which are associated to each class $\{y_i\}_{1:N}$. E.g. for sentiment classification, the prompt could be \textit{`what is the sentiment of the following review? <x>'}, where <x> is the current input $x$, (e.g.\textit{`Inception was absolutely brilliant'}), with class words \textit{bad} and \textit{good} for the negative and positive classes respectively. For a prompt classifier, $Q=\{\br{p}, \{w_i\}_{1:N} \}$, class probabilities can then be set to proportional to the probability of the associated class word, where decision $\hat{y}$ is the class with the highest probability \cite{zhao2021calibrate, jiang2020can}
% \begin{align}
%     \tilde{P}_{\theta}(y_k| \br{x}, Q) &= \frac{P_{\theta}(w_k|\br{p}(\br{x}))}{\sum_{w_i} P_{\theta}(w_i|\br{p}(\br{x})) } \label{eq:baseline} \\
%     \hat{y} &= \underset{k}{\text{argmax}} \; \tilde{P}_{\theta}(y_k|\br{x}, Q)
%     \label{eq:argmax}
% \end{align}

% \noindent Though this system could be used to return class probabilities, as a large language model, the prompt-based classifier may return probabilities that 
% are influenced by distributional statistics of words \cite{gardner2021competency, liusie-etal-2022-analyzing}. This may lead to inherent class bias, since label words may have a high probability because they have a high LM prior given the prompt, and not because they better answer the task. \\

% \noindent\textbf{Optimal Weights} To account for this, one can define re-weighting parameters $\bm{\alpha} = \{\alpha_i \}_{1:N}$, where each $\alpha_i \in \mathbb{R}^+$ scales the probabilities of the classifier, 
% \begin{align}
%     \hat{P}_{\theta}(y_k| \br{x}, Q, \bm{\alpha}) = \frac{\alpha_k \tilde{P}_{\theta}(y_k| \br{x}, Q)}{\sum_i \alpha_i \tilde{P}_{\theta}(y_i| \br{x}, Q)}
% \end{align}

% \noindent Given labelled task dataset $\mathcal{D}=\{(\br{x}^{(j)}, y^{(j)})\}_{j=1}^M$, one can then find the optimal weights $\bm{\alpha}^*$ that maximises the accuracy of the prompt classifier $\hat{P}_{\theta}(y_k| \br{x}, Q, \bm{\alpha})$ over the dataset, 
% \begin{align}
%     %\text{acc}(Q, \bm{\alpha}, \mathcal{D}) &= \sum_j \mathbbm{1}(\argmax{y} \hat{P}_{\theta}(y_k| \br{x}^{(j)}, Q, \bm{\alpha}), y^{(j)}) \\ 
%     \bm{\alpha}^* &= \argmax{\bm{\alpha}} \text{Accuracy}(Q, \bm{\alpha}, \mathcal{D}) \label{eq:optimal}
% \end{align}

% \begin{table*}[h!]
%     \centering
%     \begin{tabular}{ccc|cccccc}
%         \toprule
%         method  & inputs & labels & imdb & rt & amazon & snli & mnli & qqp \\
%         \midrule
%         baseline       & \xmark & \xmark & 85.4\std{12.7} & 78.8\std{14.0} & 86.0\std{13.8} & 45.2\std{13.7} & 43.5\std{11.3} & 65.4\std{14.0} \\ 
%         %null-norm-text      & 91.1\std{3.6}  & 88.3\std{3.5} & 94.3\std{2.8} & 60.2\std{14.4} & 55.9\std{12.2} &  \\
%         null-norm & \xmark & \xmark & 92.1\std{3.2}  & 89.1\std{3.8}  & 95.0\std{1.8}  & 75.2\std{10.4} & 66.1\std{9.7} & 77.4\std{6.6} \\
%         %prob-norm & 91.2\std{8.1} & 90.1\std{2.0} & 95.3\std{1.4} & 74.1\std{11.3} & 68.5\std{9.2} \\
%         %monte-norm      & 92.9\std{3.1}  & 90.9\std{1.6}  & 95.9\std{0.7}  & 77.9\std{9.5} & 69.8\std{9.4} & 78.3\std{2.5}\\
%         prior-match & \cmark & \xmark & 93.1\std{3.3} & 90.9\std{1.6} & 96.0\std{0.8} & 78.5\std{9.3} & 69.8\std{9.7} & 79.1\std{2.4}\\
%         optimal& \cmark & \cmark & 93.5\std{2.7} & 91.2\std{1.5}   & 96.1\std{0.7} & 79.4\std{8.2} & 70.8\std{8.6} & 82.3\std{2.8}\\
%         \bottomrule
%     \end{tabular}
%     \caption{Average dataset accuracy and standard deviations, over all prompts and label words. \textbf{baseline} and \textbf{null-norm} are zero-resource classification methods, \textbf{prior matching} uses the text inputs but not labels, while \textbf{optimal} is an oracle approach that uses the labels to search for the best thresholds.}
%     \label{tab:task_table}
% \end{table*}

% \noindent \noindent\textbf{Prior-Matching} The previous approach requires labelled data, which may limit the benefit of using prompt-based classifiers. As an alternative, one can find the values $\bar{\bm{\alpha}}$ that ensure that the classifier is unbiased, such that the class prior $\hat{P}(y_k|Q, \bm{\alpha})$, 
% \begin{align}
%     \hat{P}(y_k|Q, \bm{\alpha}) &= \mathbb{E}_{\br{x}} \{ \hat{P}(y_k|\br{x}, Q, \bm{\alpha})\} \\
%     &\approx \frac{1}{N} \sum_{j=1}^N  \hat{P}(y_k^{(j)}|\br{x}^{(j)}, Q, \bm{\alpha})
% \end{align}

% \noindent matches the true prior $P(y_k)$
% \begin{equation}
%     \bar{\bm{\alpha}} = \argmin{\bm{\alpha}} \sum_{\forall y_k} | \hat{P}(y_k|Q, \bm{\alpha}) - P(y_k)| \label{eq:unbiased}
% \end{equation}

% \noindent A deterministic solution that exactly matches the distributions exists, which can be found with a search with 1 degree of freedom (that can be accounted for by setting $\alpha_1 = 1$). If there is no expected class bias, one can assume equal probabilities over all classes, $P(y_k) = \mathcal{U}(y_k) = \frac{1}{N}$. This approach is therefore unsupervised and only requires text inputs $\mathcal{D}_{x}=\{\br{x}^{(j)}\}_{j=1}^M$, which therefore can be applied at inference to any test set. \\

% \noindent \textbf{Null-Input Approximation} The dependence of prior-matching on unlabelled dataset $\mathcal{D}_{x}$ is a drawback and may not always be available.  In Appendix \ref{sec:proof_1}, we prove that an analytical approximation of $\bar{\bm{\alpha}}$ can be made,
% \begin{equation}
%     \bar{\alpha}_k \approx \frac{1}{\mathbb{E}_{x}\{ P(w_k|\br{x}, Q) \}} = \frac{1}{P(w_k| Q)} \label{eq:monte-norm}
% \end{equation}

% \noindent Inspired by \citet{zhao2021calibrate}, we consider a resource-free approximation of the word prior (equation \ref{eq:monte-norm}) by considering the output word probabilities of the null input $\emptyset$ (i.e. an empty string). 
% \begin{align}
%     P_{\theta}(w_k | Q)  &\approx  P_{\theta}(w_k|\br{p}(\emptyset)) \label{eq:null_norm}
% \end{align}

% \noindent This enables a zero-resource approximation of reweighting parameters $\bar{\bm{\alpha}}$.

% \section{Experiments}
% \subsection{Experimental Setup}
% \noindent\textbf{Data} 
% Experimental results are run on standard NLP benchmarks, including sentiment classification (\textit{IMDB} \cite{maas-etal-2011-learning}, \textit{Rotten Tomatoes} \cite{pang-lee-2005-seeing} and \textit{amazon}), natural language inference (\textit{SNLI} \cite{bowman-etal-2015-large} and \textit{MNLI} \cite{williams-etal-2018-broad}) and paraphrase detection (\textit{QQP} \cite{wang-etal-2018-glue}). Evaluation is reported on standard test sets, except for amazon polarity where 5000 test examples were randomly sampled. \\

% \noindent\textbf{Models} We use FLAN-T5 large\footnote{https://huggingface.co/google/flan-t5-large} \cite{chung2022scaling}, a T5 with further instruction-tuning stage where the system was trained in a multi-task fashion over 1,836 tasks, each prepended with a natural instruction prompt. This work evaluates FLAN-T5 for different NLP tasks with arbitrary prompting set ups. For each task, we select 6 prompt templates and for binary classification tasks consider 25 possible class words pairs, while for NLI we have 64 class word triplets (where all permutations of valid class words are considered). All prompts and label words used are given in Appendix \ref{sec:example_prompts}. \\

% \noindent\textbf{Methods} We consider 4 different methods to leverage LLM probabilities for classification. Class word probability via equation \ref{eq:baseline} (\textbf{baseline}). Normalised probabilities calculated using null-inputs priors via equation \ref{eq:null_norm} (\textbf{null-norm}). Optimising $\alpha_k$ with a search to have unbiased class prior via equation \ref{eq:unbiased} (\textbf{prior-match}). The oracle upper-bound performance, found by optimising the optimal accuracy threshold via equation \ref{eq:optimal} (\textbf{optimal}). 

% \subsection{Experimental Results}
% \begin{figure*}[ht!]
%     \centering
%     \includegraphics[width=\linewidth]{figures/wide_box_plots/rt.png}
%     \caption{boxplots of the accuracy of all label-word pairs for \textbf{rotten tomatoes}, over all the considered prompts}
%     \label{fig:boxplot_rt}
% \end{figure*}

% % \begin{table*}[h]
% %     \centering
% %     \begin{tabular}{c|cccc}
% %         \toprule
% %         dataset  & baseline & null-norm & marg-norm & optimal threshold \\
% %         \midrule
% %         IMDB    &  \\
% %         RT      &  \\
% %         amazon  &  \\
% %         SNLI    &  \\
% %         MNLI    &  \\
% %         QQP     &  \\
% %     \end{tabular}
% %     \caption{Caption}
% %     \label{tab:my_label}
% % \end{table*}

% \noindent\textbf{Classification Robustness} Table \ref{tab:task_table} shows the mean and standard deviation of accuracies among all prompt and class word settings for a given task. We observe large consistent gains from both re-weighting approaches, with prior-matching increasing baseline accuracy by between 6.7\% to 12.1\% for sentiment classification, 13.7\% for qqp, and over 25\% for natural language inference. Prior-matching also demonstrates performance very similar to the oracle upper-bound, often within 1\%, showing that the unsupervised prior-match approach is competitive with the supervised threshold search. Prior-matching also performs better than null-norm by a small margin in all tasks, where this small gap confirms that the word-prior normalisation is a very reasonable zero-shot approximation. \\

% \noindent\textbf{Prompt Robustness} Figure \ref{fig:boxplot_rt} illustrates a boxplot of rotten tomatoes performance over all class-words for each considered method, over all 6 prompts. As observed in Table \ref{tab:task_table}, naively using raw label word probabilities (dark blue) leads to considerable fluctuations in accuracy; some prompt 
% and label word settings lead to reasonable accuracy (92\%+ accuracy), however there is observed brittleness to label word choice, with many settings demonstrating poor performance. Prior matching (green) leads to significant robustness, with nearly all sensible settings above 85\% accuracy. We further find that, as shown in Table \ref{tab:task_table}, the unsupervised approach has accuracies very comparable to those when using optimal thresholds. 

% \noindent In Figure \ref{fig:boxplot_snli}, we consider similar boxplots for SNLI and observe larger gains through reweighting. This was as higher probabilities are often assigned to the entailment and contradiction labels words, leading to under-classification of the neutral class. We observe greater sensitivity to prompt choice and label words for snli than as observed in rotten tomatoes, even with reweighting. \\

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/wide_box_plots/snli_3.png}
%     \caption{boxplots of the accuracy of all label-word sets for \textbf{snli}, for the first 3 prompts}
%     \label{fig:boxplot_snli}
% \end{figure}

% \noindent \textbf{Weight Alignment} Figure \ref{fig:threshold_lineplot} shows a scatter plot of the weights found by the optimal threshold search $\bm{\alpha}^*$ (equation \ref{eq:optimal}), with those found from the unsupervised prior matching method $\bar{\bm{\alpha}}$ (equation \ref{eq:unbiased}) and the zero-resource word prior approximation (equation \ref{eq:null_norm}). We see a clear linear relationship between optimal and prior-match, illustrating that accounting for the marginal bias is almost equivalent with maximising accuracy, however, achieved in an unsupervised fashion. Null-norm is also well correlated with the optimal thresholds, but there is a less direct relationship. Similar linear relationships are observed also for other binary-classification tasks and prompts, as shown in Appendix \ref{sec:linear_plots} \\

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.8\columnwidth]{figures/threshold_alignment/amazon.png}
%     \caption{Scatter plot of the optimal weights $\bm{\alpha}^*$ (equation \ref{eq:optimal}) with the prior match weights $\bm{\bar{\alpha}}$ (equation \ref{eq:unbiased}) and the approximation via null-norm (equation \ref{eq:null_norm}), for all settings of prompt 1 on \textbf{amazon}}
%     \label{fig:threshold_lineplot}
% \end{figure}

% \section{Conclusions}
% This paper analyzes prompt-based classifiers and demonstrates that inherent class bias is a significant factor that influences the sensitivity of the system to prompt and label words. We propose an unsupervised approach of prior matching, which we demonstrate performs competitively to the supervised alternative of searching for optimal thresholds, while avoiding the need for labelled data. We relate prior matching with word biases, and motivate a zero-resource approach of debiasing model probabilities. We show that our methods lead to practical approaches that reduce the sensitivity to design choices such as prompts and label words.

% \newpage
% \section{Limitations}
% This work considered sentiment classification, natural language inference, and paraphrase detection, and could have been extended over a greater suite of tasks to guarantee it's effectiveness. Further, this paper ran experiments on flan-t5 large, and this work has not yet explored a larger range of prompted language models. Flan-t5 has also been instruction tuned on similar tasks, and so the findings may be limited in scenarios where known capabilities have to be elicited from models robustly. Lastly, the approximation used to motivate our zero-resource approach may not always be accurate, however, the method's good performance shows that the approximation is at least somewhat reasonable. 

% \section{Ethical Considerations}
% Though this work suggests methods to improve the robustness of prompt-based classifiers to prompts and label words, this does not imply that all design choices will work. In some set ups, the system may be ineffective and have poor generalisation over the task. Deploying machine learning classifiers in real-world classification settings has many associated risks, and careful analysis should be made before deploying such systems. 

% % Entries for the entire Anthology, followed by custom entries
% \bibliography{anthology,custom}
% \bibliographystyle{acl_natbib}

% \appendix
% \section{Derivation of Normalisation Equation}
% \label{sec:proof_1}
% For a prompt classifier $Q=\{\br{p}, \{w_i\}_{1:N} \}$, class probabilities are assumed to be proportional to the probability of the associated class word,
% \begin{align}
%     \tilde{P}_{\theta}(y_k| \br{x}, Q) &= \frac{P_{\theta}(w_k|\br{p}(\br{x}))}{\sum_{w_i} P_{\theta}(w_i|\br{p}(\br{x}))}
% \end{align}


% \noindent Given the task dataset $\mathcal{D} = \{ \{ \br{x}^{(j)}, y^{(j)} \} \}_{j=1}^M$, one can calculate the assumed prior of the prompt classifier over the output classes,
% \begin{align}
%     \tilde{P}_{\theta}(y_k|Q) &= \mathbb{E}_{\br{x}} \big{\{} \tilde{P}_{\theta}(y_k|Q, \br{x}) \big{\}} \\
%            &\approx \frac{1}{M} \sum_{j=1}^M \tilde{P}_{\theta}(y_k|Q, \br{x}^{(j)}) \\
%            &= \frac{1}{M} \sum_{j=1}^M \frac{P_{\theta}(w_k|\br{p}(\br{x}^{(j)}))}{\sum_{w_i} P_{\theta}(w_i|\br{p}(\br{x}^{(j)}))}
% \end{align}

% \noindent This can be compared to the actual prior of the task/domain,
% \begin{align}
%     P(y_k) \approx P(y_k|\mathcal{D}) &= \frac{1}{M} \sum_{j=1}^M \mathbbm{1} (y, y^{(j)})
% \end{align}

% \noindent If $\mathcal{D}$ is sufficiently large, then an unbiased classifier should have a class prior similar to that approximated via the labels. However, if they diverge, one may wish to debias the classifier by scaling class probabilities by factors $\alpha_k$,

% \begin{align}
%     \hat{P}_{\theta}(y_k| \br{x}, Q, \bm{\alpha}) &= \frac{\alpha_k \tilde{P}_{\theta}(y_k| \br{x}, Q)}{\sum_i \alpha_i \tilde{P}_{\theta}(y_i| \br{x}, Q)}
%     \\
%     &= \frac{\alpha_k P_{\theta}(w_k| \br{x}, Q)}{Z(\br{x}, Q, \bm{\alpha})}
% \end{align}


% \noindent Where $Z(\br{x}, Q, \bm{\alpha})= \sum_i \alpha_i P_{\theta}(w_i| \br{x}, Q, \bm{\alpha})$ and $P_{\theta}(w_k|\br{x}, Q) \equiv P_{\theta}(w_k|\br{p}(\br{x}))$. The parameters $\bar{\bm{\alpha}}$ that lead to an unbiased classifier can then be determined in a deterministic fashion. 
% \begin{equation}
%     \bar{\bm{\alpha}} = \argmin{\bm{\alpha}} \sum_{\forall y_k} | \hat{P}_{\theta}(y_k|Q, \bm{\alpha}) - P(y_k)|
% \end{equation}

% \noindent Note that by constraining $\alpha_1=1$, there will exist a deterministic solution that ensures that $\hat{P}_{\theta}(y_k|Q, \bm{\alpha}) = P(y_k)$. For given weight parameters $\bm{\alpha}$, Consider the prompt-classifier priors, $\hat{P}_{\theta}(y_k| Q, \bm{\alpha})$. One can approximate this using a Taylor series of the expectation of a ratio, yielding
% \begin{align}
%     \hat{P}_{\theta}(y_k| Q, \bm{\alpha}) &= \mathbb{E}_{\br{x}}[\hat{P}_{\theta}(y_k| \br{x}, Q, \bm{\alpha})]  \\
%                     &= \mathbb{E}_{\br{x}}[\frac{\alpha_k P_{\theta}(w_k| \br{x}, Q)}{Z(\br{x}, Q, \bm{\alpha})}] \\
%                     &\approx \frac{\mathbb{E}_{\br{x}}[\alpha_k P_{\theta}(w_k| \br{x}, Q)]}{\mathbb{E}_{\br{x}}[Z(\br{x}, Q, \bm{\alpha})]} \\
%                     &= \frac{\alpha_k P_{\theta}(w_k| Q)}{Z(Q, \bm{\alpha})}
% \end{align}


% \noindent By equating the predicted prior with the true prior, we find an approximation for $\bar{\bm{\alpha_k}}$
% \begin{align}
%     \hat{P}_{\theta}(y_k| Q) &= P(y_k|D) \\
%     \frac{\alpha_k P_{\theta}(w_k| Q)}{Z(Q)} &= P(y_k|D) \\
%     \Rightarrow \alpha_k &= \frac{Z(Q) \cdot P(y_k|D)}{P_{\theta}(w_k| Q)}
% \end{align}

% \noindent A final insight is that in many cases it is assumed that there should be no inherent class bias, and so $P(y_k|D)$ can be assumed to be uniform and be included in the normalisation term. 

% % \subsection{Effectiveness of Approximations}
% % \begin{table}[H]
% %     \small
% %     \centering
% %     \begin{tabular}{c|cc||cc||cc}
% %         \toprule
% %                          & bad & amazing & poor & good & negative & great \\
% %         \midrule
% %          dataset         & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0\\
% %          \midrule
% %          baseline        & 74.9 & 25.1 & 30.6 & 69.4 & 72.9 & 27.1 \\
% %          class-norm      & 69.1 & 30.8 & 36.1 & 63.9 & 68.0 & 32.0 \\
% %          monte-log-norm  & 52.2 & 47.7 & 51.1 & 48.9 & 54.1 & 45.9 \\
% %          monte-prob-norm & 56.3 & 43.7 & 46.5 & 53.5 & 53.5 & 46.5 \\
% %          null-norm       & 68.7 & 31.2 & 51.3 & 48.7 & 78.6 & 21.4 \\
% %          \bottomrule
% %     \end{tabular}
% %     \caption{Marginalised class probabilities $\hat{P}(y|Q)$ compared with dataset distribution $P(y|\mathcal{D})$ for imdb}
% %     \label{tab:my_label}
% % \end{table}

% % \subsection{Expectation}
% % I agree that 

% % \begin{equation}
% %     \frac{\hat{P}(y_1| Q)}{\hat{P}(y_2| Q)} = \frac{\hat{P}(y_1| \mathcal{D})}{\hat{P}(y_2| \mathcal{D})}
% % \end{equation}

% % But I don't believe that an equivalent statement is that:
% % \begin{equation}
% %     \mathbbm{E}_x \Big{\{} \frac{\hat{P}(y_1| Q, \br{x})}{\hat{P}(y_2| Q, \br{x})} \Big{\}} = \frac{\hat{P}(y_1| \mathcal{D})}{\hat{P}(y_2| \mathcal{D})}
% % \end{equation}

% % As to satisfy this the system must output that $\hat{P}(y_1| Q, \br{x}) = \hat{P}(y_2| Q, \br{x})$ for all $\br{x}$. Looking at the equation, however, we see that for individual decisions the system should be able to favour specific classes and therefore the expectation is likely to be much larger than 1. 

% % \subsection{Ways to optimise $\alpha$}
% % \begin{itemize}
% %     \item Find $\alpha$s such that $\hat{P}(y_1| Q) = \hat{P}(y_1| D)$
% %     \item Find $\alpha$s that maximise accuracy 
% % \end{itemize}

% % Emperically it appears that the two are equivalent

% \section{Prompts and Label Words}
% \label{sec:example_prompts}
% \subsection{Sentiment Classification}
% \begin{table}[H]
%     \small
%     \centering
%     \begin{tabular}{l}
%         \toprule
%         \multicolumn{1}{c}{prompt}           \\
%         \midrule
%         classify the following review:       \\
%         how was the movie?                   \\
%         which word best describes the text?  \\
%         what is the sentiment?               \\
%         what is the reviewer's verdict?      \\
%         is the following movie good or bad?  \\
%         \bottomrule
%     \end{tabular}
%     \caption{sentiment classification prompts}
%     \label{tab:temp}
% \end{table}

% \begin{table}[H]
%     \small
%     \centering
%     \begin{tabular}{l|l}
%         \toprule
%         positive  & negative    \\
%         \midrule
%         good         & bad        \\
%         great        & terrible   \\
%         amazing      & poor       \\
%         fantastic    & horrible   \\
%         positive     & negative   \\
%         \bottomrule
%     \end{tabular}
%     \caption{label words for sentiment classification}
%     \label{tab:temp}
% \end{table}

% \subsection{Natural Language Inference}
% \begin{table}[H]
%     \small
%     \centering
%     \begin{tabular}{l}
%         \toprule
%         \multicolumn{1}{c}{prompt}                             \\
%         \midrule
%         is the second text an entailment of the first text?        \\
%         does the second text directly follow from the first text?  \\
%         are the texts related?                                     \\
%         are the texts consistent?                                  \\
%         does text 1 imply text 2?                                  \\
%         can text 2 be logically derived from text 1?               \\
%         does the hypothesis logically follow the premise?          \\
%         \bottomrule
%     \end{tabular}
%     \caption{NLI prompts}
%     \label{tab:temp}
% \end{table}

% \begin{table}[H]
%     \small
%     \centering
%     \begin{tabular}{l|l|l}
%         \toprule
%         entailment  & neutral & contradiction     \\
%         \midrule
%         yes         & maybe       & no            \\
%         correct     & unclear     & incorrect     \\
%         yeah        & potentially & nope          \\
%         follows     & neutral     & contradiction \\
%         \bottomrule
%     \end{tabular}
%     \caption{label words for NLI}
%     \label{tab:temp}
% \end{table}

% \subsection{Paraphrase Identification}
% \begin{table}[H]
%     \small
%     \centering
%     \begin{tabular}{l}
%         \toprule
%         \multicolumn{1}{c}{prompt} \\
%         \midrule
%         is the second text a paraphrase of the first text?        \\
%         are the two texts semantically equivalent?  \\
%         are the texts paraphrases of each other? \\
%         do the texts have the same meaning? \\
%         is the meaning of text 1 the same as in text 2? \\
%         would the two texts be classified as paraphrases?  \\
%         \bottomrule
%     \end{tabular}
%     \caption{NLI prompts}
%     \label{tab:temp}
% \end{table}

% \begin{table}[H]
%     \small
%     \centering
%     \begin{tabular}{l|l}
%         \toprule
%         paraphrase  & not paraphrase    \\
%         \midrule
%         yes       & no        \\
%         correct   & incorrect   \\
%         yeah      & not       \\
%         positive  & negative   \\
%         true      & false   \\
%         \bottomrule
%     \end{tabular}
%     \caption{label words for sentiment classification}
%     \label{tab:temp}
% \end{table}

% \section{further Threshold Alignment plots}
% \label{sec:linear_plots}
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.8\columnwidth]{figures/threshold_alignment/rt.png}
%     \caption{weights alignment plot for \textbf{rotten tomatoes}}
%     \label{fig:boxplot_imdb}
% \end{figure}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.8\columnwidth]{figures/threshold_alignment/imdb.png}
%     \caption{weights alignment plot for \textbf{imdb}}
%     \label{fig:boxplot_imdb}
% \end{figure}

% \onecolumn
% \section{Further Boxplots}
% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=\linewidth]{figures/wide_box_plots/imdb.png}
%     \caption{boxplots of the accuracy of all label-word pairs on \textbf{IMDB}, over all the considered prompts}
%     \label{fig:none}
% \end{figure}

% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=\linewidth]{figures/wide_box_plots/amazon.png}
%     \caption{boxplots of the accuracy of all label-word pairs on \textbf{amazon}, over all the considered prompts}    \label{fig:none}
% \end{figure}

% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=\linewidth]{figures/wide_box_plots/qqp.png}
%     \caption{boxplots of the accuracy of all label-word pairs on \textbf{qqp}, over all the considered prompts}    \label{fig:none}
% \end{figure}

% \end{document}

% \onecolumn
% \section{Reworking of Maths}
% LMs model the probabilities distribution over possible output sequences, $P_{\theta}(\br{w}|\br{x})$. For input $\br{x}\in\mathcal{X}$, a prompt $\br{p}$ reformats the input text into a prompted template of the input, $\br{p}(\br{x})\in\mathcal{X}$. For classification tasks with classes $\{y_i\}_{1:N}$, assume a set of words associated with particular task classes, $\{w_i\}_{1:N}$. Class probabilities are then assumed to be proportional to the probability of generating the associated class word
% \begin{align}
%     P(y_k| \br{x}, Q) &= \frac{P_{\theta}(w_k|\br{p}(\br{x}))}{\sum_{w_i} P_{\theta}(w_i|\br{p}(\br{x})) }
% \end{align}

% \noindent Where Q is the realisation of the prompt classifier, comprising of the classifier target words $\{w_i\}_{i=1:N}$ and prompt $\br{p}$- both selected to be compatible for the task $\mathcal{T}$. \\

% \noindent Assume that a training/development dataset $\mathcal{D}$ is available for the task,
% \begin{align}
%     \mathcal{D} = \{ \{ \br{x}^{(j)}, y^{(j)} \} \}_{j=1}^N 
% \end{align}

% \noindent One can calculate the assumed prior of the prompt classifier over the output classes,
% \begin{align}
%     P(y_k|Q) &= \mathbb{E} \big{\{} P(y_k|Q, \br{x}) \big{\}}_{\br{x}\sim P( \br{x}|\mathcal{T})} \\
%            &\approx \frac{1}{N} \sum_{j=1}^N P(y_k|Q, \br{x}^{(j)}) \\
%            &= \frac{1}{N} \sum_{j=1}^N \frac{P_{\theta}(w_k|\br{p}(\br{x}^{(j)}))}{\sum_{w_i} P_{\theta}(w_i|\br{p}(\br{x}^{(j)}))}
% \end{align}

% \noindent Which can be compared to the actual prior of the training domain,
% \begin{align}
%     P(y_k|\mathcal{D}) &= \frac{1}{N} \sum_{j=1}^N \delta (y, y^{(j)})
% \end{align}

% \noindent Where $\delta$ is the kronecker delta function. Assuming that the dataset $\mathcal{D}$ is sufficiently large, then an unbiased classifier should lead to a similar class prior to that approximated via the labels. However, if they largely diverge, then one may wish to debias the classifier by scaling class probabilities by factors $\alpha_k$, yielding an unbiased classifier $\hat{P}(y_k| \br{x}, Q)$,
% \begin{align}
%     \hat{P}(y_k| \br{x}, Q) = \frac{\alpha_k P(y_k| \br{x}, Q)}{Z(\br{x}, Q)}
% \end{align}

% \noindent Where the normalisation term $Z(\br{x}, Q)$ is required to ensure that $\hat{P}(y_k| \br{x}, Q)$ is a valid distribution. Note that
% \begin{align}
%     \hat{P}(y_k| Q) &= \mathbb{E}[\hat{P}(y_k| Q, \br{x})]_{x \sim P(x|\mathcal{T})} \\
%                     &= \mathbb{E}[\frac{\alpha_k P(y_k| \br{x}, Q)}{Z(\br{x}, Q)}]  \\
%                     &\approx \frac{\mathbb{E}[\alpha_k P(y_k| \br{x}, Q)]}{\mathbb{E}[Z(\br{x}, Q)]} \\
%                     &= \frac{\alpha_k P(y_k| Q)}{Z(Q)}
%                     % &= \frac{1}{N} \sum_{j=1}^N \hat{P}(y_k|Q, \br{x}^{(j)}) \\
%                     % &= \frac{1}{N} \sum_{j=1}^N \alpha_k P(y_k|Q, \br{x}^{(j)}) \\ 
%                     % &= \alpha_k P(y_k| Q)
% \end{align}

% \noindent therefore by matching the predicted prior with the true prior, we can find an approximation for $\alpha_k$
% \begin{align}
%     \hat{P}(y_k| Q) &= P(y_k|D) \\
%     \frac{\alpha_k P(y_k| Q)}{Z(Q)} &= P(y_k|D) \\
%     \Rightarrow \alpha_k &= \frac{1}{Z(Q)} \cdot \frac{P(y_k|D)}{P(y_k| Q)}
% \end{align}

% \noindent Leading to the (approximately) unbiased posterior, 
% \begin{align}
%      \hat{P}(y_k| \br{x}, Q) = \frac{1}{Z(Q)} \cdot \frac{P(y_k|D)}{P(y_k| Q)} \cdot P(y_k| \br{x}, Q) 
% \end{align}


% \noindent For classification, the highest class is selected. In the binary case this can be done by looking at the posterior ratio, 
% \begin{align}
%     \frac{\hat{P}(y_1| \br{x}, Q)}{\hat{P}(y_0| \br{x}, Q)} = \frac{P(y_1| \br{x}, Q)}{P(y_0| \br{x}, Q)} \cdot \frac{P(y_0| Q)}{P(y_1| Q)}
% \end{align}

% \noindent Where if the posterior ratio is greater than 1 then $\hat{y}=1$, and otherwise $\hat{y}=0$. This leads to the following decision rule:
% \begin{align}
% \hat{y} = \begin{cases}
% 			1 & \text{if} \quad \frac{P(y_1| \br{x}, Q)}{P(y_0| \br{x}, Q)} \ge \frac{P(y_1| Q)}{P(y_0| Q)}\\
%             0 & \qquad \qquad \text{otherwise}
% 		 \end{cases}
% \label{eq:thresh_norm}
% \end{align}


% \noindent We know consider ways of estimating the ratio $\frac{P(y_1| Q)}{P(y_0| Q)}$. It was previously stated that the word prior could be estimated as:
% \begin{align}
%     P(y_k|Q) &= \mathbb{E} \big{\{} P(y_k|Q, \br{x}) \big{\}}_{\br{x}\sim P( \br{x}|\mathcal{T})} \\
%     &= \mathbb{E} \Big{\{} \frac{P_{\theta}(w_k|\br{p}(\br{x})}{\sum_{w_i} P_{\theta}(w_i|\br{p}(\br{x}))} \Big{\}}_{\br{x}\sim P( \br{x}|\mathcal{T})} \\
%     &\approx \frac{1}{N} \sum_{j=1}^N \frac{P_{\theta}(w_k|\br{p}(\br{x}^{(j)}))}{Z_j}
% \end{align}

% \noindent Where $Z_j = \sum_{w_i} P_{\theta}(w_i|\br{p}(\br{x}^{(j)}))$. These expressions cannot be used to simplify $\frac{P(y_1| Q)}{P(y_0| Q)}$ due to the $Z_j$'s within the summation. However, we can make the following assumption:
% \begin{align}
%     P(y_k|Q) &= \mathbb{E} \Big{\{} \frac{P_{\theta}(w_k|\br{p}(\br{x})}{\sum_{w_i} P_{\theta}(w_i|\br{p}(\br{x}))} \Big{\}}_{\br{x}\sim P( \br{x}|\mathcal{T})} \\
%             &\approx \frac{ \mathbb{E} \{ P_{\theta}(w_k|\br{p}(\br{x}) \}}{ \mathbb{E} \{ \sum_{w_i} P_{\theta}(w_i|\br{p}(\br{x})) \}} \\
% \end{align}



% if we consider the geometric mean by taking the expectation of log probability, 
% \begin{align}
%     \log P(y_k|Q) &= \mathbb{E} \big{\{} \log P(y_k|Q, \br{x}) \big{\}}_{\br{x}\sim P( \br{x}|\mathcal{T})} \\
%     &= \mathbb{E} \Big{\{} \log P_{\theta}(w_k|\br{p}(\br{x})) - \log \sum_{w_i} P_{\theta}(w_i|\br{p}(\br{x})) \Big{\}}_{\br{x}\sim P( \br{x}|\mathcal{T})} \\
%     &\approx \frac{1}{N} \sum_{j=1}^N \log P_{\theta}(w_k|\br{p}(\br{x}^{(j)})) - \frac{1}{N} \sum_{j=1}^N \log Z^{(j)}
% \end{align}

% \noindent Then the probability ratio can be simplified in terms of the word's average log probabilities:
% \begin{align}
%     \log \frac{P(y_1| Q)}{P(y_0| Q)} &= \mathbb{E} \Big{\{} \log P_{\theta}(w_1|\br{p}(\br{x})) - \log P_{\theta}(w_0|\br{p}(\br{x})) \Big{\}}_{\br{x}\sim P( \br{x}|\mathcal{T})} 
%     \\
%     \frac{P(y_1| Q)}{P(y_0| Q)} &\approx \exp \Big{(} \frac{1}{N} \sum_{j=1}^N \log P_{\theta}(w_1|\br{p}(\br{x}^{(j)})) - \log P_{\theta}(w_0|\br{p}(\br{x}^{(j)})) \Big{)} \\
% \end{align}


% \noindent This can be compared to the optimal decision threshold, $\tau$, that maximises the accuracy for the task data.

% \begin{align}
% \hat{y} = \begin{cases}
% 			1 & \text{if} \quad \frac{P(y_1| \br{x}, Q)}{P(y_0| \br{x}, Q)} \ge \tau\\
%             0 & \qquad \text{otherwise}
% 		 \end{cases}
% \label{eq:thresh_norm}
% \end{align}


% \section{Extra Results}
% \section{Limitations}



==> scratch_2.tex <==
Given an input sequence, LMs model the probability distribution over possible output sequences, $P_{\theta}(\br{w}|\br{x})$. For classification tasks, a prompt-based classifier comprises of the prompt  $\br{p}$ which reformats the input text $\br{x}\in\mathcal{X}$ to $\br{p}(\br{x})\in\mathcal{X}$, and class words $\{w_i\}_{1:N}$ which are associated to each class $\{y_i\}_{1:N}$. E.g. for classification, the prompt could be \textit{`what is the sentiment of the following movie? <x>'} (where <x> is the current input $x$, e.g.\textit{`Inception was absolutely brilliant'}), with class words \textit{bad} and \textit{good} for the negative and positive classes respectively. For a prompt classifier, $Q=\{\br{p}, \{w_i\}_{1:N} \}$, class probabilities are then assumed to be proportional to the probability of the associated class word, where decision $\hat{y}$ is the class with the highest probability \cite{zhao2021calibrate, jiang2020can}
\begin{align}
    P(y_k| \br{x}, Q) &= \frac{P_{\theta}(w_k|\br{p}(\br{x}))}{\sum_{w_i} P_{\theta}(w_i|\br{p}(\br{x})) } \\
    \hat{y} &= \underset{k}{\text{argmax}} \; P(y_k|\br{x})
    \label{eq:argmax}
\end{align}

As a general-purpose LLM, the system should ideally demonstrate good performance for most sensible settings $Q$. However, a possible issue is that as a language model, the prompt-based classifier has likely learned distributional statistics over words \cite{gardner2021competency, liusie-etal-2022-analyzing}. Certain words may have a higher probability, not because they better answer the task, but because they have a larger prior given the prompt. To determine if this is the case, given a dataset $\mathcal{D} = \{ \{ \br{x}^{(j)}, y^{(j)} \} \}_{j=1}^N$, one can estimate the prior over the output classes, $P(y_k|Q)$, and compare this to the true prior, $P(y_k|\mathcal{D})$

\begin{align}
    P(y_k|Q) &\approx \frac{1}{N} \sum_{j=1}^N P(y_k|Q, \br{x}^{(j)}) \\
             &= \frac{1}{N} \sum_{j=1}^N \frac{P_{\theta}(w_k|\br{p}(\br{x}^{(j)}))}{\sum_{w_i} P_{\theta}(w_i|\br{p}(\br{x}^{(j)}))} \\
    P(y_k|\mathcal{D}) &= \frac{1}{N} \sum_{j=1}^N \delta (y, y^{(j)})
\end{align}

Where $\delta$ is the delta function. If the estimates in equation 3 and equation 5 largely diverge, then one can define an unbiased classifier, $\hat{P}(y_k| \br{x}, Q)$, as
\begin{align}
     \hat{P}(y_k| \br{x}, Q) = \frac{P(y_k|D)}{P(y_k| Q)} \cdot P(y_k| \br{x}, Q) 
\end{align}

